Crayon: Customized On-Device LLM via Instant Adapter Blending and Edge-Server Hybrid Inference

The customization of large language models (LLMs) for user-specified tasks gets important. However, maintaining all the customized LLMs on cloud servers incurs substantial memory and computational overheads, and uploading user data can also lead to privacy concerns. On-device LLMs can offer a promising solution by mitigating these issues. Yet, the performance of on-device LLMs is inherently constrained by the limitations of small-scaled models. To overcome these restrictions, we first propose Crayon, a novel approach for on-device LLM customization. Crayon begins by constructing a pool of diverse base adapters, and then we instantly blend them into a customized adapter without extra training. In addition, we develop a device-server hybrid inference strategy, which deftly allocates more demanding queries or non-customized tasks to a larger, more capable LLM on a server. This ensures optimal performance without sacrificing the benefits of on-device customization. We carefully craft a novel benchmark from multiple question-answer datasets, and show the efficacy of our method in the LLM customization.

==> app/03_various_arch.tex <==
\section{Various On-device LLM}
\label{sec:app:various}

\begin{table}[t]
  \centering
  \begin{adjustbox}{width=\linewidth}
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    \multirow{2}{*}{on-device LLM}  & \multicolumn{2}{c}{7B} &  \multicolumn{2}{c}{13B} & \multirow{2}{*}{\alg (7B)} \\
    % \cmidrule(ll){2-3} \cmidrule(ll){4-5}
     & zero-shot & few-shot & zero-shot & few-shot & \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule{6-6}
    LLaMA-2& 39.6 & 44.4 & 50.7 & 55.6& 45.5\\
    Mistral& 59.3 & 60.1 & n/a & n/a & \\
\bottomrule
    
    \end{tabular}
    \end{adjustbox}
  \caption{\textbf{Various on-device LLMs.} In terms of accuracy (\%), we compare the proposed \alg with various on-device LLMs such as LLaMA-2 and Mistral. }
  \label{tab:various_llm}
\end{table}


To validate the efficacy of \alg to various on-device LLMs, we apply our proposed method to LLaMA-2~\cite{touvron2023llama2} and Mistral~\cite{jiang2023mistral}. As shown in \autoref{tab:various_llm}, \alg shows a performance gap of more than 1.1\% compared to the performance of the same sized on-device LLMs. In conclusion, Crayon is applicable to a variety of on-device LLMs and proves improved performance.

==> contents/01_intro_bak.tex <==
\section{Introduction} 

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/main_figure.pdf}

    \caption{\textbf{Overall design of \alg.} To overcome the performance limits of on-device LLM, we devise the method generating a suitable adapter instantly by utilizing an adapter palette. Our method can be splitted as three folds; preparation of an adapter palette, generation of personalized adapter, and device-server hybrid inference. For more details, see in \autoref{sec:method}.}
    \label{fig:intro}
\end{figure*}

Large language models (LLMs) have achieved unprecedented success on diverse natural language processing (NLP) tasks such as machine translation, question and answering, text summarization and stylization, etc. To make the better use of the versatility of LLM, several services such as GPTs~\cite{gpts} and PersonaAI~\cite{characterai, meta_gen} have been emerged to specialize the LLMs to a specific user's request, i.e. \textit{personalization}.

Due to the significantly large size of LLM, keeping all the users' personalized LLMs in the servers imposes a tremendous burden. Then, the focus is shifting towards \textit{on-device LLM.} Under the limited computing power of edge devices, it is impractical to address models as large as those on the servers. Therefore, for on-device LLM personalization, it is crucial to maintain the performance on user-defined tasks, while lightening the model size. The practical method for the on-device LLM personalization, however, has been less explored.
% However, how to realize the on-device LLM personalization is understudied.


Recently, several works are developed to further lead out the ability of LLMs, and they may be exploited to cover the performance limit of LLMs on smaller size (device-level). \citet{brown2020language} introduced few-shot learning where a few example query-answer prompts are given together with users' queries. Chain-of-thought (COT)~\cite{wei2022chain} tried in-context learning by encouraging LLM to generate evidences as well as final answers. Also, for knowledge-intensive NLP tasks, retrieval augmented generation (RAG)~\cite{lewis2020retrieval} made up query-relevant prompts by retrieving a given database. These prompt-based approaches have a intrinsic problem of increasing inference cost as the prompts get long and complex, and hence they are not suitable for edge devices.

Moreover, we can consider fine-tuning the on-device LLM in order to internalize these prompt-based knowledge for user-specific tasks to the model. Freezing the pre-trained LLM, adapter-based methods~\cite{hu2021lora,houlsby2019parameter,wang2022adamix} have tried to facilitate LLM fine-tuning, and the low-rank-based adapter LoRA~\cite{hu2021lora} have been most in the limelight. Despite on-device-scale LLM armed with the adapters, %fine-tuning still needs huge computational cost and datasets, 
fine-tuning is time-consuming process and also needs a certain-level of training dataset. However, computing power of edge devices is limited and collecting enough personal data is also impractical. Accordingly, we raise the idea:  \textit{How about simply personalizing LLM with no additional training on-device?}

To this end, we propose a method personalizing the on-device LLM via a single personalized adapter which is blended on-the-fly from a set of base adapters given a target personalization task (few sample queries of a user). As depicted in~\autoref{fig:intro}, our approach requires no additional training cost in both of server and edge device when deploying the personalized adapter. In addition, we develop a device-server hybrid inference strategy to effectively leverage the better-generalized larger model of the server for handling unexpected queries (out-of-scope for the personalized model). In a nutshell, our contributions are summarized as follows:

\begin{comment}
Large Language Model (LLM) has shown the significant performance improvement for multiple natural language tasks such as language translation, Question and Answering, etc. Accordingly, some chatbot applications have been emerged to answer the users' requests, and many researchers have tried their best to update their model with frequent cycles to beat the other LLMs. 


Despite of giving the significant satisfaction to users, the LLM service has a big burden to maintain due to high computational cost of LLM. Hence, deploying the LLM to the end device is inevitable to reduce the computational costs in the server. Due to limited computational power on the end device, the on-device model(\ie sLLM) should be smaller than the server-sided model(\ie LLM), and thus it occurs the performance degradation. 

To alleviate declined performance, the authors in~\cite{brown2020language} introduced \code{few-shot learning} by adding several pairs of questions and answers which are similar to the users' query into prompts, and they showed that few-shot learning has better performance for most of the tasks than zero-shot learning. Moreover, Chain-of-Thought~\cite{wei2022chain} validated the performance enhancement for several tasks by getting answers and reasons from LLMs, and thus in-context learning has crucial role to improve the performance. 
Furthermore, by expanding on in-context learning, retrieval augmented generation (RAG)~\cite{lewis2020retrieval} was firstly introduced for knowledge-intensive NLP tasks. It selects the relevant data in terms of the users' query from the users' database, and add those data into the prompts before inference. However, those kinds of prompting-based approaches have a intrinsic problem of increasing inference cost, and thus it is not applicable for on-device.

Lastly, finetuning sLLM is one of the option to improve the performance for the target task. Since updating all the weights of sLLM still needs huge computational costs and datasets, the authors~\cite{hu2021lora} proposed low rank adapter (LoRA) that is one of the parameter efficient finetuning methods. Different from above two approaches, this approach does not require the additional inference cost but require training. To train the LoRA that is suitable for a user's interest, it is necessary to prepare the server and the user's private data, but it is hard to be gathered and utilized by the legal issue of privacy. Under this circumstance, we can raise the idea: \textit{How about generating personalized LoRA from pre-trained LoRA models without additional training?}
 
% Under this circumstance, we can raise the research question: \textit{Can several pre-trained LoRAs cover the unseen task without additional training?}

To solve our inquiry, we propose \alg that is generating a personalized LoRA instantly by using pretrained LoRA pools and a few number of user's data without additional training as shown in \autoref{fig:intro}. Our contributions are summarized as follows: 
\end{comment}

\begin{itemize}
    \item We propose the first practical approach for personalization of on-device small-scale LLM.
    % \item \jt{We suggest a practical approach for personalization of on-device smaller-scale LLM, for the fist time.}
    \item We first jointly learn a pool of LLM adapters, constraining their diversification, and then generate a personalized adapter instantly via blending the pre-defined adapter pool.
    \item We also develop a device-server harmonic inference to fill the performance gap between personalized and non-personalized tasks.
    \item We construct an LLM personalization benchmark by tailoring the diverse public question-answer datasets for quantitative evaluation.
    %\item \jh{We firstly propose the framework that generates a personalized adapter instantly via blending a pool of pre-defined adapters.} %As such, latency of our method is almost zero maintaining higher performance than naive LoRA tuning.
    % so that the users can change their LoRA instantaneously when their interested task is changed. 
    %\item \jh{We propose the joint training method for multiple adapters under task-undefined dataset to have positive synergy among them.}
    %\item \jh{We suggest a \textit{device-server hybrid inference strategy} in order to mitigate the low-quality responses from the on-device model when confronted with unexpected queries.}
\end{itemize}


